Distributed peer review enhanced with natural language processing and machine learning

While ancient scientists often had patrons to fund their work, peer review of proposals for the allocation of resources is a foundation of modern science. A very common method is that proposals are evaluated by a small panel of experts (due to logistics and funding limitations) nominated by the grant-giving institutions. The expert panel process introduces several issues - most notably: 1) biases introduced in the selection of the panel. 2) experts have to read a very large number of proposals. Distributed Peer Review promises to alleviate several of the described problems by distributing the task of reviewing among the proposers. Each proposer is given a limited number of proposals to review and rank. We present the result of an experiment running a machine-learning enhanced distributed peer review process for allocation of telescope time at the European Southern Observatory. In this work, we show that the distributed peer review is statistically the same as a `traditional' panel, that our machine learning algorithm can predict expertise of reviewers with a high success rate, and we find that seniority and reviewer expertise have an influence on review quality. The general experience has been overwhelmingly praised from the participating community (using an anonymous feedback mechanism).

==> discussion.tex <==
\section{\label{sec:disc}Discussion}

In this paper, we study a novel way of peer review which distributes the task among the proposers. We trialled several enhancements to the `classic' distributed peer review process. We used natural language processing -- specifically the \dt framework -- to infer the domain expertise of the reviewers and distributed proposals accordingly. We also asked the proposers to evaluate the helpfulness of the comments giving us an additional statistics.

\begin{comment}
Such a process has many advantages. The workload of refereeing is distributed which allows the allocation of more referees to each proposal. This can reduce the statistical fluctuation in proposal evaluation \citep[see for instance][]{2018PASP..130h4501P}.

The process also involves very junior researchers in the proposal selection process. They can contribute their expertise (especially as they are often very close to research) without massively affecting the process. This also trains future science leaders early in judging other scientists' work with a positive learning effect for both their own science as well as for mentoring their future students.  The aim is to find if such a We have tested various aspects of this experiment. 

We find that the self-selected participants follow a very similar \fpa{what did you want to say here?}
\end{comment}

\subsection{Distributed Peer Review vs Classical TAC}

Once two independent bodies reviewing the same set of applications have provided their final rankings, there is no known metric based on the rankings to judge which of the two is better.
In the case of telescope time allocation, one would need to implement both recommendations and then evaluate the scientific impact of the two selections (with all its limitations - specifically a missing objective way to quantify ``impact''). This a-posteriori way of quantifying the quality of the reviews would require multiple experiments and large investments in terms of time -- an infeasible endeavour.


Therefore, the comparison between different review processes has to rely on different criteria, accounting for the fact that subjectivity plays a very important role.
Although instances in which the same set of applications was submitted to two or more panels are rare (because they are typically expensive), the few published cases show that the typical agreement in the top quartile is $\sim$50\%, while in the central quartiles this decreases to about 33\% (see P18 and references therein). This suggests that a better approach to evaluate review processes is to ask whether two different panels are characterised by the same level of subjectivity. Or, put in a more quantitative way, how the two reviews compare in terms of their internal consistency (through the agreement fractions). In this framework, the DPR review and the pre-meeting OPC review show the same level of internal consistency (see Section~\ref{sec:analysis.opcomp}). This indicates that the single referees behave in a similar way in the two implementations.

The cross-reviews DPR-OPC agreement being smaller than the internal DPR-DPR agreement (see Section~\ref{sec:analysis.opcomp.agfrac}) is not unexpected, as there are intrinsic differences between the two setups (see Section~\ref{sec:analysis.opcomp}). Very importantly,
the \dt DPR matches proposals to the reviewers by estimating their expertise (see details in the method description of the supplementary material) for the given proposal. This procedure,
which makes use of natural language processing, is much more fine-grained and objective than the self-reported science classification of the OPC process (see Section~\ref{sec:eso}).

\begin{comment}
The cross-reviews DPR-OPC agreement being smaller than the internal DPR-DPR agreement (see Section~\ref{sec:analysis.opcomp.agfrac}) is not unexpected. There are intrinsic differences of the two setups: The OPC panel members are selected from a more senior pool. As a result, the panels are composed by about 88\% of senior scientists, and only 12\% of senior postdocs (from the second post-doc onward; no PhD students). The DPR composition reflects the distribution of the users community (see \ref{sec:analsysis.demo}), with 27.2\% of the reviewers being junior scientists (with no PhD and/or at less than 4 years from the PhD). 
%\fpa{Not sure it is good to mention this here, as we concluded that the junior people do not affect the process. So, I would drop from "the OPC panel members are selected" onward.}
A further difference is that the \dt DPR matches proposals to the reviewers by estimating their expertise (see Section~\ref{sec:reviewer_selection}) for the given proposal. This is much more fine-grained and objective way using natural language processing when compared to the self-reported science classification of the OPC process. The automated way. 
\end{comment}

The largest difference between the two processes discussed here is the absence of a face-to-face meeting in the DPR implementation. However, it is unclear whether the panel discussions lead to the selection of better science. As discussed previously there is currently no objective criteria for measuring ``better science''. However, several studies have shown that the meeting increases the differences between two panels with respect to the pre-meeting agreement. In other words, while it increases the internal consensus by polarizing different opinions within the panels, it does not lead to a better panel-panel agreement (see \citealt{Obrecht2007} and references therein). This might indicate that a face-to-face meeting does not make the process better. This point will be addressed in greater detail in P19.

\subsection{Deployment Scenarios for \dt DPR}

Gemini has already implemented a variant of this mechanism successfully over the past years under the moniker Fast Turnaround \citep{Gemini}\footnote{See also: \url{http://staff.gemini.edu/ft/}}. The approach presented in this work enhances this process using better review-proposal matching based on natural language processing. The next logical step is to expand this experiment and distribute a fraction of observing time using DPR at more facilities. More than 95\% of the participants suggest an implementation of such a scheme (see statistics in the feedback section of the supplementary material) for some part of the ESO proposal categories.

\begin{comment}
\begin{figure}
   \includegraphics[width=0.5\textwidth]{plots/stats_application_of_dpr.pdf}
   \caption{\label{fig:application_of_dpr}The participant was asked the question \textit{For which types of proposals do you think distributed peer review would be beneficial?}}
\end{figure}
\end{comment}

The example of the Gemini ``Fast Turnaround''-channel has prompted ESO to consider a similar fast track channel that would get time allocation through DPR. When explicitly asked about the deployment of the DPR for the Fast Track Channel, only $\sim$15\% of the users declared to be concerned about this proposition (see statistics in the feedback section of the supplementary material).

The coupling of the machine learning \dt back-end with DPR allows a deployment of such a fast track with (bi) monthly calls using relatively few resources while still ensuring expert reviews. 


\subsection{Machine Learning for Review Processes}
\label{sec:conclusion.ml}
The presented work shows the promising application of machine learning (in particular natural language processing) on review processes \citep[see also][]{2017AJ....153..181S}. This first attempt already has a remarkable accuracy (see Figure~\ref{fig:dt_vs_ref_knowledge}) using a relatively simple metric. There are several other more complex algorithms (e.g. using author position when constructing the knowledge vectors) that can now be tested against the given data. 

\begin{comment}
% this figure is used twice, identical (FPA, commented out)
\begin{figure}
   \includegraphics[width=0.5\textwidth]{plots/stats_time_spent_expertise.pdf}
   \caption{\label{fig:time_spent_expertise}The referee was asked the question \textit{Was the time spent for proposals for which you are an expert versus a non-expert different?}}
\end{figure}
\end{comment}


This, however, is only the beginning of applying such techniques in the review process. Potentially, using author overlap and similarity of papers, it might be feasible to automatically identify competing groups and mutually exclude them from reviewing each other's proposals. Machine Learning can also be applied to flag unhelpful comments already in the review stage - prompting the reviewer to improve them. This is just one of the many possible enhancements to make the review process more effective and easier. 

\subsection{Bias and Confidentiality}
\label{sec:conclusion.bias_confidentiality}
As for the confidentiality, this is of course a delicate matter, which is of the utmost importance. Like in the classic panel scheme, it cannot be policed a priory, and it can only rely on the integrity of the reviewers, who all sign the non-disclosure agreement. Here we can only add that in the case of the Fast Turnaround implemented at the Gemini Telescopes, the reported misbehaviour is at the level of less than one per mill (Kissler-Patig, private communication). This is in line with what is seen in the regular OPC process at ESO. Although more data will need to be accumulated to properly quantify this potential issue, at the moment there is no reason to believe that the DPR would show a misbehaviour rate that is higher than in the classical process. Future deployments of the DPR framework, might allow to indicate reviewers that should be excluded for a specific proposal (machine learning - as discussed in Section~\ref{sec:conclusion.ml} - might help with that as well).
In this respect it is worth noting that less than 30\% of them declared to be more concerned about confidentiality issues in the DPR process than in the OPC process (see the statistics question on confidentiality in the supplementary material).

\begin{comment}
\begin{figure}
   \includegraphics[width=0.5\textwidth]{plots/stats_bias_robustness.pdf}
   \caption{\label{fig:bias_robustness}The referee was asked the question \textit{Robustness of the review process against any biases:}}
\end{figure}

\begin{figure}
   \includegraphics[width=0.5\textwidth]{plots/stats_confidentiality_concern.pdf}
   \caption{\label{fig:confidentiality_concern}The referee was asked the question \textit{Securing confidentiality in the process:}}
\end{figure}
\end{comment}


==> long_analysis.tex <==
\section{\label{sec:analysis} Analysis}

There are a myriad statistics available that can be interesting to apply to the dataset (some of them are explored in the supplementary material). We therefore encourage the community to make use the anonymized dataset to run independent analyses. Our main focus in this study is to address two questions: 1) How well can our knowledge vectors predict expertise for a proposal? 2) How different is the DPR from a more traditional \gls{eso.opc} review. We were also interested in possible differences in the way experts and ``non-experts'' judge a proposal.



\subsection{Domain Knowledge Inference}
\label{sec:analysis.knowledge_vectors}
\begin{figure}[h!]
   \includegraphics[width=\columnwidth]{plots/knowledge_group_vs_ref_knowledge.pdf}
   \caption{Conditional probability $P(\textrm{self reported}|\textsc{DeepThought})$ for the various combinations of perceived and \dt inferred knowledge.}
   \label{fig:dt_vs_ref_knowledge}
\end{figure}
We aim to predict the expertise of a referee when related to a given proposal using objective criteria. "Expertise" is, unfortunately, no such criterion. However, it is reasonable to assume that the self-judgement of expertise (self-efficacy) is a good measure that might approximate such a quantity relatively well.

Given:
\begin{itemize}
    \item ``self reported'' as the self reported domain knowledge 
    \item \textsc{DeepThought} as the \textsc{DeepThought} inferred domain knowledge 
\end{itemize}
For our experiment, we calculate the joint probability $P(\textrm{Self Reported}|\textsc{DeepThought})$ using Bayes theorem:

\begin{align}
   P(\textrm{Self Reported}&|\textsc{DeepThought}) =\\ 
   &\frac{P(\textsc{DeepThought}|\textrm{Self Reported})P(\textrm{Self Reported})}{P(\textsc{DeepThought})}\nonumber
\end{align}
\begin{align}
   P(\textrm{Self Reported}|&\textsc{DeepThought}) =\\ 
   &\frac{P(\textsc{DeepThought})\cap(\textrm{Self Reported})}{P(\textsc{DeepThought})}\nonumber
\end{align}

Figure~\ref{fig:dt_vs_ref_knowledge} shows the correlation between self reported knowledge (see the detailed description of the experiment in the supplementary material) and our predicted DeepThought inferred knowledge (see supplementary material for a detailed description of the method). The correlation is very high with only few outliers.

\subsection{Expertise influence on Review}

An important question is whether expertise has an influence on the review process itself. 

Statistics shows that experts take tentatively less time to review proposals than non-experts (see supplementary material for statistics). 

\begin{comment}
\begin{figure}
   \includegraphics[width=0.5\textwidth]{plots/stats_time_spent_expertise.pdf}
   \caption{\label{fig:time_spent_expertise}The referee was asked the question \textit{Was the time spent for proposals for which you are an expert versus a non-expert different?}}
\end{figure}

Figure~\ref{fig:non_expert_review_satisfaction} shows that non-expert reviewers were able to review the proposals but in general did not feel very confident about their task. 

\begin{figure}
   \includegraphics[width=0.5\textwidth]{plots/stats_non_expert_review_satisfaction.pdf}
   \caption{\label{fig:non_expert_review_satisfaction}The referee was asked the question \textit{How satisfactorily were you able to evaluate the proposals for which you were a non-expert?}}
\end{figure}
\end{comment}

We also study how expertise influences the grade distribution. Figure~\ref{fig:dt_vs_ref_grade_violin} shows that the difference in the shapes related to experts and referees with little to no domain knowledge is relatively small. The distributions show an extended tail towards poor grades, similarly to what is seen in Figure~4 of \citet{2018PASP..130h4501P} for the large OPC sample.



In their study on the effects of reviewer expertise on the evaluation of funding applications, \citet{2016PLoSO..1165147G} concluded that "reviewers with higher levels of self-assessed expertise tended to be harsher in their evaluations". That study was based on a sample of 1044 reviewers, i.e. 6 times larger than ours. Although our data may contain some indication of this trend, the differences are statistically marginal.

\begin{figure*}[t]
   \includegraphics[width=\columnwidth]{plots/dt_knowledge_group_vs_grade.pdf}
   \includegraphics[width=\columnwidth]{plots/ref_knowledge_vs_grade.pdf}
   \caption{The distribution of grades for different groups of referees. The horizontal lines mark quartiles. \textbf{Left:} The distribution of grades for the different groups domain knowledge inferred by the \dt algorithm. \textbf{Right:} The distribution of grades for the different groups of self-reported domain knowledge.}
   \label{fig:dt_vs_ref_grade_violin}
\end{figure*}


\subsection{Rating the helpfulness of Review comments}

After the review process, we asked the proposers to evaluate the ``helpfulness'' of the review comments. A total of 136 reviewers provided feedback.

The review usefulness distribution shows a steady rise, with a sudden drop off at the `very helpful' bin (see subfigures in Figure~\ref{fig:review_review_overview}). About 55\% of the users rated the comments in the `helpful' and `very helpful' bins.

%The Review of the review follows a similar distribution than the review of the %proposal Figure~\ref{fig:review_review_overview} shows a stetig steigende?? %distribution with a sudden drop off to the ``highest'' grade of `very helpful'.
\begin{comment}
\begin{figure}
   \includegraphics[width=\columnwidth]{plots/review_review_overview.pdf}
   \caption{Distribution of the ``helpfulness'' rating for the referee provided comments for the entire sample.\wek{move to appendix}}
   \label{fig:review_review_overview}
\end{figure}
\end{comment}

For checking what factors might influence the ability to write helpful comments we use the same statistical method given in Section~\ref{sec:analysis.knowledge_vectors}.

The first test is to see how the comment's helpfulness is being evaluated given a certain quartile that the proposal uses $P(\textrm{helpful comment}|\textrm{proposal quartile})$. This shows a similar distribution to Figure~\ref{fig:review_review_overview}. There are some small differences. Comments for proposals second to the top quartile often were perceived as relatively helpful. Comments to proposals in the last quartile were rarely ranked as very helpful. 

The reviewer's expertise is expected to have an influence on the helpfulness of comments. The upper row in Figure~\ref{fig:review_review_overview} shows both the influence of perceived knowledge and \dt inferred knowledge on the helpfulness of the comment. The probabilities are very similar between the perceived and inferred knowledge. We highlight that experts seemingly very rarely give unhelpful comments and that non-experts rarely give very helpful comments. 


We checked whether seniority has an influence on the ability of creating helpful comments. Figure~\ref{fig:review_review_overview} shows some correlation between the seniority and the ability for the referee to give helpful comments. Most interesting is the inability of graduate students to give very helpful comments. This might be a training issue and can be resolved by exposing the students to schemes like DPR.


We have also asked about the helpfulness of the comment in our general feedback (see supplementary materiak). The distribution of comment usefulness follows the distribution of helpfulness for individual comments relatively closely (see statistics in the supplementary material).

The comments given in the DPR compare very favourable when compared to the \gls{eso.opc} (see details in the supplementary materials)).
\begin{comment}
\begin{figure}
   \includegraphics[width=0.5\textwidth]{plots/stats_helpful_comments.pdf}
   \caption{The referee was asked the question \textit{How useful were the comments that you received on your proposal?}}
   \label{fig:helpful_comments}
\end{figure}


\begin{figure}
   \includegraphics[width=0.5\textwidth]{plots/stats_comment_opc_compare.pdf}
   \caption{The referee was asked the question \textit{How do these raw comments compare to the edited comments from the OPC in the past?}}
   \label{fig:comment_opc_compare}
\end{figure}
\end{comment}

\begin{figure*}[ht!]
   \includegraphics[width=\columnwidth]{plots/review_review_dt_knowledge_vs_rating.pdf}
   \includegraphics[width=\columnwidth]{plots/review_review_ref_knowledge_vs_rating.pdf}
   \includegraphics[width=\columnwidth]{plots/review_review_seniority_vs_rating.pdf}
   \includegraphics[width=\columnwidth]{plots/review_review_prop_rank_vs_rating.pdf}


   \caption{\textbf{Upper Row:} Evaluation of the helpfulness of the comment given expertise (inferred by  \dt on the left panel and self reported on the right panel). 
   \textbf{Lower Left:} We show the conditional probability $P(\textrm{helpful comment}|\textrm{gender})$ for the various combinations of helpful comment rating and reported gender.
   \textbf{Lower Right:}We show the conditional probability $P(\textrm{helpful comment}|\textrm{proposal quartile})$ for the various combinations of helpful comment rating and proposal quartile.}
   \label{fig:review_review_overview}
\end{figure*}

\subsection{Feedback to the DPR}
\label{sec:analysis.feedback}

We summarize here the feedback provided by the participants on the 5 free-form questions (see the detailed questions and statistics in the supplementary material) in the questionnaire circulated after the experiment. The general feedback to the experiment was overwhelmingly positive.

While technical improvements like automatic saving were suggested, overall the usability of the software was praised (see statistics in the supplementary material). A repeated suggestion is to stream-line the reviewing process by having a grade for each of the assessment criteria and require a minimum amount of words in the written feedback. Another returning suggestion is to fully anonymise the proposal (including for example removing the previous use of ESO facilities) as well as to leave out the time requested (so that reviewers focus even better on judging only the science). 

By far the most and strongest raised suggestion was to restrict as much as possible to expert reviewers. Many respondents, when acting as a non-expert reviewer, felt uncomfortable and tended to give average grades. On the receiving end, they prefer to know for each of the provided assessments the expert level of the reviewer and possibly have their grade weighted accordingly. Along the same lines, the suggestion was to use DPR for a first selection, but then still have a panel assessing the remaining proposals while taking into the account the DPR results as 'external reviews'. Even so, nearly all people are positive about DPR and many mentioned explicitly how the evaluation of other proposals as well as the received (unfiltered) feedback will help to improve their own proposals.

\section{Comparison of DeepThought DPR with OPC}
\label{sec:analysis.opcomp}

The proposals used in the DPR experiment were also reviewed through the regular ESO OPC channel. This allows a comparison between the outcomes of the two processes. However, these differ by construction in many aspects, and so a one-to-one comparison is not possible. This is because in the DPR experiment:

\begin{enumerate}
\item there is no a-priory scientific-seniority selection;
\item the proposals are typically reviewed by $N_r>6$ referees (while $N_r=3$ in the pre-meeting OPC process);
\item the number of proposals per referee is much smaller;
\item the set of proposals common to different reviewers is much smaller;
\item there is no triage;
\item there is no face-to-face discussion.
\end{enumerate}

Bearing these caveats in mind, in the following we will discuss various aspects of the comparison.


\subsection{\label{sec:analysis.opcomp.subpanel}The sub-panel agreement fraction}  

A robust way of quantifying the consistency between two different panels reviewing the same set of proposals is that of the quartile agreement fraction introduced in \citet[][hereafter P18]{2018PASP..130h4501P} (Section~9.2). Following that concept, one can compute what we will indicate as the panel-panel (p-p) quartile agreement matrix (QAM). The generic QAM element $M_{i,j}$ is the fraction of proposals ranked by the first panel in the $i$-th quartile of the grade distribution, that were ranked in the $j$-th quartile by the second panel.
If we indicate with $A_i$ and $B_j$ the events "a proposal is ranked by panel A in quartile $i$" and "a proposal is ranked by panel B in quartile $j$", the QAM elements represent the conditional probability:

\begin{displaymath}
M_{i,j}=P(A_i | B_j) = \frac{P(A_i \cap B_j)}{P(A_j)}.
\end{displaymath}

For a completely aleatory process $P(A_i \cap B_j)=P(A_i) P(B_j)$, and therefore all the terms of the QAM would be equal to 0.25, while for a full correlation, all terms would be null, with the exception of the diagonal terms, which would be equal to 1. We note that the matrix elements are not independent from each other as, by definition:

\begin{displaymath}
\sum_i M_{i,j} \equiv \sum_j M_{i,j} \equiv 1.
\end{displaymath}

While we will use this concept in the comparison with the OPC (see next section), here we will adopt it to quantify the level of subjectivity in the DPR review. For this purpose, and following the idea presented in P18 (Section~6.4), we compute the agreement fractions between pairs of sub-sets of reviews within the DPR sample. In a first test, for each of the 172 proposals we extract a random pair of reviews, which are then used to produce two rank-lists, from which the QAM is derived. The process is then repeated a large number of times, leading to the construction of an average QAM and the standard deviation matrix. Since this is constructed for simple reviewer pairs, we will indicate it as the referee-referee (r-r) QAM. The result is presented in Table~\ref{tab:rrqam} for the calibrated grades (very similar values are obtained using the raw grades). The typical standard deviation of single realizations is 0.06, while the uncertainty on the average values is below 0.01.

\begin{table}
\caption{\label{tab:rrqam}Bootstrapped DPR r-r QAM.}
\tabcolsep 5.0mm
\centerline{
\begin{tabular}{c|cccc}
\hline
\hline
 1st referee.  & \multicolumn{4}{c}{2nd referee Quartile}\\
 quartile & 1 & 2 & 3 & 4\\
\hline
1 & 0.33 &  0.26 & 0.24 &  0.18\\
2 & 0.26 &  0.26 & 0.25 &  0.23\\
3 & 0.24 &  0.25 & 0.25 &  0.26\\
4 & 0.18 &  0.23 & 0.26 &  0.34\\
\hline\hline
\end{tabular}
}
\end{table}

The values are statistically indistinguishable from those reported in P18 (Table~2) for the OPC sample including $\sim$15,000 proposals. This shows that the average r-r agreement is identical in the two processes. On average, the ranking lists produced by two distinct referees have about 33\% of the proposals in common in their first and last quartiles. This corresponds to a Cohen's kappa coefficient $k$=0.11 \citep{cohen1960}. In the central quartiles the intersection is compatible with a purely random selection. This extends to the mixed cases ($i \neq j$), with the exception of the extreme quartiles: the fraction of proposals ranked in the first quartile by one referee and in the fourth quartile by another referee is $\sim$18\%, which deviates in a statistically significant way from the random value ($k=-$0.28). No meaningful difference is seen in the QAMs computed for the OPC-Emulate (OE; 60 proposals) and Deep-Thought (DT; 112 proposals) sub-samples.

As a further test, we have investigated the possible dependence on the scientific seniority level. In the feedback questionnaire we asked the participants to express it in terms of the years after PhD, specified within 4 groups (0=no PhD; 1=less than 4 years; 2=between 4 and 12; 3: more than 12). Of the 167 reviewers, 136 provided this information, which we used to divide the reviewers in two classes: junior (groups 0 and 1) and senior (groups 2 and 3). These classes roughly correspond to PhD students plus junior post-docs (37), and advanced post-docs plus senior scientists (99). We then computed the r-r QAM for the two classes. The first quartile terms are 0.22 and 0.32 for the two classes, respectively. At face value this indicates a larger agreement between senior reviewers. However, the small size of the junior class produces a significant scatter, and therefore we do not attach too much confidence to this result.


One can extend the above bootstrapping procedure to sub-sets with a number of referees $N_r>$1. Particularly interesting is the case of $N_r=$3, because this is directly comparable to the results presented in P18. The procedure is as follows. We first make a selection of the proposals having at least 6 reviews (164). For each of them we randomly select two distinct (i.e. non-intersecting) sub-sets of $N_r$=3 grades each, from which two average grades are derived. The subsequent steps are identical to the r-r procedure, and lead to what we will indicate as the panel-panel (p-p) QAM.

The results are shown in Table~\ref{tab:ppqam}. The first-quartile agreement is about 40\% ($k$=0.21), while for the second and third quartile this is $\sim$30\%. The top-bottom quartile agreement is 10\% ($k=-$0.60).

\begin{table}
\caption{\label{tab:ppqam}Bootstrapped DPR p-p QAM ($N_r$=3).}
\tabcolsep 5.0mm
\centerline{
\begin{tabular}{c|cccc}
\hline
\hline
 1st sub-p.  & \multicolumn{4}{c}{2nd sub-panel Quartile}\\
 quartile & 1 & 2 & 3 & 4\\
\hline
1 & 0.41 &  0.29 & 0.21 &  0.10\\
2 & 0.30 &  0.30 & 0.25 &  0.16\\
3 & 0.20 &  0.24 & 0.30 &  0.25\\
4 & 0.10 &  0.18 & 0.27 &  0.45\\
\hline\hline
\end{tabular}
}
\end{table}

These values are very similar to those presented in P18 for the OPC process for $N_r$=3 sub-panels (Table~3 therein). As for the r-r case, the OE and DT sub-samples yield statistically indistinguishable values. Finally, the numbers derived from the bootstrap procedure fully agree with the results presented in P18 for different panel sizes. For $N_r$=1, 2, and 3 the first quartile agreement fractions are 0.34, 0.37 and 0.41, respectively. These match (within the noise) the corresponding P18 values (Table~8): 0.33, 0.39 and 0.45.

The conclusion is that, in terms of self-consistency, the DPR review behaves in the same way as the pre-meeting OPC process.
        
        
\subsection{\label{sec:analysis.opcomp.agfrac}The DPR-OPC agreement fraction}     

As anticipated, the proposals used in the DPR experiment were also subject to the regular OPC review. This enables the comparison between the outcomes of the two selections, with the caveats outlined above about their inherent differences.

For a first test we used a bootstrap procedure in which, for each proposal included in the DPR, we randomly extracted one evaluation from the DPR (typically one out of 7) and one from the OPC (one out of 3), forming two ranking lists from which a QAM was computed. The operation was repeated a large number of times and the average and standard deviation matrices were constructed. This approach provides a direct indication of the DPR-OPC agreement at the r-r level, and overcomes the problem that the two reviews have a different number of evaluations per proposal (see below). The result is presented in Table~\ref{tab:dpropc1to1}. The typical standard deviation of single realizations from the average is 0.06.

\begin{table}
\caption{\label{tab:dpropc1to1}DPR-OPC (pre-meeting) r-r QAM.}
\tabcolsep 5.0mm
\centerline{
\begin{tabular}{c|cccc}
\hline
\hline
 DPR ref.  & \multicolumn{4}{c}{OPC referee quartile}\\
 quartile & 1 & 2 & 3 & 4\\
\hline
1 & 0.31 &  0.26 & 0.24 &  0.18\\
2 & 0.24 &  0.27 & 0.25 &  0.24\\
3 & 0.24 &  0.23 & 0.26 &  0.26\\
4 & 0.20 &  0.23 & 0.25 &  0.31\\
\hline\hline
\end{tabular}
}
\end{table}

This matrix is very similar to that derived within the DPR reviews (Table~\ref{tab:rrqam}), possibly indicating a DPR-OPC r-r agreement slightly lower than the corresponding DPR-DPR. A check run on the two sub-samples for the junior and senior DPR reviewers (according to the classification described in the previous section) has given statistically indistinguishable results.

As explained in the introduction, the proposals were reviewed by $N_r$=3 OPC referees in the pre-meeting phase. This constitutes a significant difference, in that the DPR ranking is typically based on $\sim$7 grades, whilst the pre-meeting OPC ranking rests on 3 grades only. With this caveat in mind, one can nevertheless compute the QAM for the two overall ranking lists.

 The result (computed using calibrated grades) is presented in Table~\ref{tab:qampre}. At face value, about 37\% of the proposals ranked in the 1st quartile by the DPR were ranked in the same quartile by the OPC, with a similar fraction for the bottom quartile. When looking at these values, one needs to consider that this is only one realization, which is affected by a large scatter, as one can deduce from the comparatively large fluctuations in the QAM. These are evident when comparing, for instance, to the average values obtained from the bootstrapping procedures described in the previous section; or considering that the average matrix is expected to be symmetric.

        
\begin{table}
\caption{\label{tab:qampre}DPR-OPC (pre-meeting) p-p QAM.}
\tabcolsep 5.0mm
\centerline{
\begin{tabular}{c|cccc}
\hline
\hline
 DPR  & \multicolumn{4}{c}{OPC quartile}\\
 quartile & 1 & 2 & 3 & 4\\
\hline
1 & 0.37 &  0.26 & 0.28 &  0.09\\
2 & 0.28 &  0.16 & 0.28 &  0.28\\
3 & 0.16 &  0.40 & 0.19 &  0.26\\
4 & 0.19 &  0.19 & 0.26 &  0.37\\
\hline\hline
\end{tabular}
}
\end{table}
     
To quantify the expected noise on a single panel-panel realization, we have run a set of simulations along the lines described in P18, which are based on the statistical description of the reviewers and on the True Grade Hypothesis (see P18; Section~7 therein). For the purposes of this analysis we modified the original code to allow the calculation of the QAM for pairs of panels with different sizes. We emphasize that the P18 code was designed to simulate the OPC process, i.e. it deals with panels reviewing the same set of proposals which, in turn, are reviewed by all referees in the panels. It therefore does not fully reproduce the DPR side, in which each proposal is reviewed by a virtually different panel in the \dt sub-sample. For this reason the results should be considered only as indicative. More sophisticated simulations will be presented elsewhere.

The outcome is presented in Table~\ref{tab:qampresim} (top), which also shows the standard deviation of the single realizations (bottom). For the DPR simulated panels we have used $N_r$=7, which is close to the actual average number of reviewers per proposal in the experiment. For the OPC we have set $N_r$=3.
The numerical calculations predict a top and bottom quartile agreement of about 50\%, while in the central quartiles this drops to about 30\%. 
The statistical significance of the deviations of the observed QAM from the average QAM can be quantified using the predicted dispersion. For the first and fourth quartile, the observed value (0.37) differs at the 1.3$\sigma$-level from the average value. For the central quartiles the difference is at the $\sim$1.5$\sigma$-level. 

Therefore, although lower than expected on average, the observed DPR-OPC agreement is statistically consistent with that expected from the statistical description of the pre-meeting OPC process (P18).

\begin{table}
\caption{\label{tab:qampresim}Simulated p-p QAM (top) and uncertainty (bottom) for two panels with $N_r$=3 and $N_r$=7.}
\tabcolsep 5.4mm
\centerline{
\begin{tabular}{c|cccc}
\hline
\hline
 1st pan.  & \multicolumn{4}{c}{2nd panel quartile}\\
 quartile & 1 & 2 & 3 & 4\\
\hline
1 & 0.51 &  0.28 & 0.16 &  0.06\\
2 & 0.28 &  0.31 & 0.27 &  0.15\\
3 & 0.16 &  0.27 & 0.30 &  0.28\\
4 & 0.06 &  0.15 & 0.28 &  0.51\\
\hline
1 & 0.11 &  0.10 & 0.09 &  0.06\\
2 & 0.10 &  0.10 & 0.10 &  0.09\\
3 & 0.08 &  0.09 & 0.10 &  0.10\\
4 & 0.06 &  0.08 & 0.10 &  0.11\\
\hline\hline
\end{tabular}
}
\end{table}

One important aspect to remark is that, given the large noise inherent to the process, a much larger data-set (or more realizations of the experiment) would be required to reach a statistical significance sufficiently high to make robust claims about systematic deviations.

\subsection{\label{sec:analysis.opcomp.postopc}Comparison with the post-meeting outcome}

The fact that in the real OPC process there is a face-to-face meeting constitutes the most pronounced difference between the two review schemes. In the meeting, the opinions of single reviewers are changed by the discussion, so that the grades attributed by the single referees are not completely independent from each other (as opposed to the pre-meeting phase, in which the possible correlation should depend only on the intrinsic merits of the proposal).

The effects of the meeting can be quantified in terms of the quartile agreement fractions between the pre- and post-meeting outcomes, as outlined in \citet[][hereafter P19]{Patat2019}. Based on the P18 sample, P19 concludes that the change is significant: on average, only 75\% of the proposals ranked in the top quartile before the meeting remain in the top quartile after the discussion (about 20\% are demoted to the second quartile, and 5\% to the third quartile). P19 characterizes this effect introducing the Quartile Migration Matrix (QMM). For the specific case of P103, the QMM is reported in Table~\ref{tab:qmm} for the 683 proposals that passed the triage (top), and for the sub-set of the DPR experiment (bottom).\footnote{Of the initial 172 proposals included in the DPR sample, 36 were triaged out in the OPC process.} 

\begin{table}
\caption{OPC Quartile Migration Matrix}
\label{tab:qmm}
\tabcolsep 4.5mm
\centerline{
\begin{tabular}{c|cccc}
\hline
\hline
  OPC pre-m.  & \multicolumn{4}{c}{OPC post-meeting quartile (N=683)}\\
  quartile & 1 & 2 & 3 & 4\\
\hline
1 & 0.64 &  0.25 & 0.06 &  0.05\\
2 & 0.26 &  0.37 & 0.28 &  0.08\\
3 & 0.08 &  0.26 & 0.39 &  0.26\\
4 & 0.02 &  0.11 & 0.25 &  0.62\\
\hline 
  & \multicolumn{4}{c}{DPR sub-set (N=136)}\\
\hline
1 & 0.56 &  0.32 & 0.12 &  0.00\\
2 & 0.32 &  0.32 & 0.29 &  0.06\\
3 & 0.12 &  0.26 & 0.38 &  0.24\\
4 & 0.00 &  0.09 & 0.21 &  0.71\\
\hline\hline
\end{tabular}
}
\end{table}

As anticipated, the effect of the discussion is very pronounced. In the light of these facts one can finally inspect the QAM between the DPR and the final outcome of the OPC process. This is presented in Table~\ref{tab:qamfinal}. With the only possible exception of $M_{4,4}$, which indicates a relatively marked agreement for the proposals in the bottom quartile, the two reviews appear to be almost completely uncorrelated. By means of simple Monte-Carlo calculations one can show that for two fully aleatory panels the standard deviation of a single realization around the average value (0.25) is 0.10. Therefore, the majority of the $M_{i,j}$ elements in Table~\ref{tab:qamfinal} are consistent with a stochastic process at the 1$\sigma$ level.

\begin{table}
\caption{DPR vs. OPC post-meeting QAM}
\label{tab:qamfinal}
\tabcolsep 5.1mm
\centerline{
\begin{tabular}{c|cccc}
\hline
\hline
  DPR  & \multicolumn{4}{c}{OPC post-meeting quartile (N=136)}\\
quartile & 1 & 2 & 3 & 4\\
\hline
1 & 0.26 &  0.38 & 0.24 &  0.12\\
2 & 0.24 &  0.35 & 0.24 &  0.18\\
3 & 0.32 &  0.12 & 0.29 &  0.26\\
4 & 0.19 &  0.15 & 0.24 &  0.44\\
\hline \hline
\end{tabular}
}
\end{table}

The main conclusion is that while the pre-meeting agreement is consistent with the DPR and OPC reviewers behaving in a very similar way (in terms of r-r and p-p agreements), the face-to-face meeting has the effect of significantly increasing the discrepancy between the two processes.
We remark that the sample is relatively small, and therefore the results are significantly affected by noise.

